Self-Supervised Learning for Time Series Analysis: Taxonomy, Progress, and Prospects

Self-supervised learning (SSL) has recently achieved impressive performance on various time series tasks. The most prominent advantage of SSL is that it reduces the dependence on labeled data. Based on the pre-training and fine-tuning strategy, even a small amount of labeled data can achieve high performance. Compared with many published self-supervised surveys on computer vision and natural language processing, a comprehensive survey for time series SSL is still missing. To fill this gap, we review current state-of-the-art SSL methods for time series data in this article. To this end, we first comprehensively review existing surveys related to SSL and time series, and then provide a new taxonomy of existing time series SSL methods by summarizing them from three perspectives: generative-based, contrastive-based, and adversarial-based. These methods are further divided into ten subcategories with detailed reviews and discussions about their key intuitions, main frameworks, advantages and disadvantages. To facilitate the experiments and validation of time series SSL methods, we also summarize datasets commonly used in time series forecasting, classification, anomaly detection, and clustering tasks. Finally, we present the future directions of SSL for time series analysis.

==> 11_biographies.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/zhangkexin.eps}}]
{Kexin Zhang} received the B.S. and the M.S. degrees in engineering from China University of Geosciences, Wuhan, China, in 2016 and 2019, respectively,  and the Ph.D. degree in control engineering and science from Zhejiang University, Hangzhou, China in 2023. His major research interests include intelligent time series analysis, deep learning, data-driven industrial fault diagnosis, and artificial intelligence security.
\vspace{-10pt}
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/QingsongWen.jpg}}]
{Qingsong Wen} (SM'23) is the Head of AI Research \& Chief Scientist at Squirrel Ai Learning. Previously, he worked at Alibaba, Qualcomm, and Marvell. He received his M.S. and Ph.D. degrees in Electrical and Computer Engineering from Georgia Institute of Technology, Atlanta, USA. He has published over 80 top-ranked conference and journal papers, received AAAI/IAAI 2023 Innovative Application Award, and won the First Place in 2022 ICASSP Grand Challenge Competition. He co-organized the Workshop on AI for Time Series (at KDD 2023, IJCAI 2023, ICDM 2023, SDM 2024, AAAI 2024). He is an Associate Editor for Neurocomputing, Guest Editor for IEEE Internet of Things Journal, Guest Editor for Applied Energy, and regularly served as an Area Chair/SPC/PC member of the major AI conferences including AAAI, IJCAI, KDD, ICDM, ICASSP, etc. His research interests include AI for time series, AI for education, and general machine learning.
\vspace{-20pt}
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/chaoli.jpg}}]
{Chaoli Zhang} received the B.S. degree in information security from Nankai University, China, in 2015, and the Ph.D. degree in computer science and engineering from Shanghai Jiao Tong University, China in 2020. She is currently a lecturer with the School of Computer Science and Technology, Zhejiang Normal University. She engaged in research at Alibaba DAMO Academy for nearly three years. Her research interests include time series analysis, algorithmic game theory and mechanism design, networking. She won the gold prize of ICASSP-SPGC root cause analysis for wireless network fault localization 2022. She was the recipient of Google Anita Borg Scholarship 2014 and AAAI/IAAI innovative deployed application award 2023. 
\vspace{-20pt}
\end{IEEEbiography}


\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/cairongyao.jpg}}]
 {Rongyao Cai} received the B.S. degress in chemical engineering from Zhejiang University of Technology, Hangzhou, China, in 2022. He is studying for the M.S. degree in control engineering with College of Control Science and Engineering, Zhejiang University, Hangzhou, China. His major research interests include data mining, machine learning on industrial time-series data.
 \vspace{-20pt}
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/mingjin.jpg}}]{Ming Jin} 
received the B.Eng. degree from the Hebei University of Technology, Tianjin, China, in 2017, and M.Inf.Tech. degree from the University of Melbourne, Melbourne, Australia, in 2019. He is currently pursuing his Ph.D. degree in Computer Science at Monash University, Melbourne, Australia. His research focuses on graph neural networks (GNNs), time series analysis, data mining, and machine learning. 
\vspace{-20pt}
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/liuyong.eps}}]
{Yong Liu} (M'11) received the B.S. degree in computer science and engineering and the Ph.D. degree in computer science from Zhejiang University, Hangzhou, China, in 2001 and 2007, respectively. He is currently a Professor with the Institute of Cyber Systems and Control, Department of Control Science and Engineering, Zhejiang University. He has authored or co-authored more than 30 research papers in machine learning, computer vision, information fusion, and robotics. His current research interests include machine learning, robotics vision, information processing, and granular computing.
\vspace{-20pt}
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/jamesbio.eps}}]
{James Y. Zhang} is the managing director of AI Forecast and Strategy Platform of Ant Group.  Prior to his employment with Ant Group, he worked on finance-related AI at Bloomberg, spearheaded the creation of Bloomberg's GPU computation farm and participated in the establishment of the AI branch of Bloomberg Labs.  He obtained his Ph.D. degree from the Univ. of Ottawa, Canada, in Electrical Engineering in 2006, and both his Master’s and Bachelor's degrees from Zhejiang Univ., China, in 2000 and 1997, respectively.
His industrial experience of startups and larger corporations spans various disciplines, such as image processing, natural language processing, time series analysis, high-speed hardware development, optical networks, operations research, biometrics, and financial systems, with extensive patents and publications.
\vspace{-20pt}
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Yuxuan.jpg}}]{Yuxuan Liang} is currently an Assistant Professor at Intelligent Transportation Thrust, also affiliated with Data Science and Analytics Thrust, Hong Kong University of Science and Technology (Guangzhou). He is working on the research, development, and innovation of spatio-temporal data mining and AI, with a broad range of applications in smart cities. Before that, he obtained his PhD degree at National University of Singapore. He published over 50 peer-reviewed papers in refereed journals and conferences, such as TPAMI, TKDE, AI Journal, TMC, KDD, WWW, NeurIPS, and ICLR. Three of them were selected as the most influential IJCAI/KDD papers. He received The 23rd China Patent Excellence Award in 2022.
\vspace{-20pt}
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/GuansongPang.png}}]
{Guansong Pang} is a tenure-track Assistant Professor of Computer Science in the School of Computing and Information Systems at Singapore Management University (SMU), Singapore. Before joining SMU, he was a Research Fellow with the Australian Institute for Machine Learning (AIML). He received a Ph.D. degree from University of Technology Sydney, Australia in 2019. His research interests lie in machine
learning techniques and their applications, with a focus on handling abnormal and unknown data.
\vspace{-20pt}
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.3in,clip,keepaspectratio]{figures/DongjinSong.jpg}}]
{Dongjin Song} received a Ph.D. degree from University of California San Diego (UCSD) in 2016. Currently, he is an assistant professor in the School of Computing at the University of Connecticut (UConn). His research interests include machine learning, deep learning, data mining, and related applications for time series data and graph representation learning. Papers describing his research have been published at top-tier data science and artificial intelligence conferences, such as NeurIPS, ICML, ICLR, KDD, ICDM, SDM, AAAI, IJCAI, CVPR, ICCV, etc. He has co-organized AI for Time Series (AI4TS) workshop at IJCAI 2022, 2023 and the Mining and Learning from Time Series workshop at KDD 2022, 2023. He has also served as senior PC for AAAI, IJCAI, and CIKM. He won the UConn Research Excellence Research (REP) Award in 2021. His research has been funded by NSF, USDA, Morgan Stanley, NEC Labs America, Travelers, etc.
\vspace{-20pt}
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/shirui-bio.jpg}}]{Shirui Pan} received a Ph.D. in computer science from the University of Technology Sydney (UTS), Ultimo, NSW, Australia. He is a Professor with the School of Information and Communication Technology, Griffith University, Australia.
Prior to this, he was a Senior Lecturer with the Faculty of IT at Monash University. 
His research interests include data mining and machine learning. To date, Dr Pan has published over 100 research papers in top-tier journals and conferences, including TPAMI, TKDE, TNNLS, ICML, NeurIPS, and KDD. His research has attracted over 20,000 citations. His research received the 2024 CIS IEEE TNNLS Oustanding Paper Award and the 2020 IEEE ICDM Best Student Paper Award. He is recognized as one of the AI 2000 AAAI/IJCAI Most Influential Scholars in Australia (2021). He is an ARC Future Fellow and a Fellow of Queensland Academy of Arts and Sciences (FQA).
\vspace{-20pt}
\end{IEEEbiography}

==> 9_acknowledgement.tex <==
\section*{Acknowledgment}
The authors would like to thank...
